Specifications: The missing link to making the development of LLM systems an engineering discipline

Despite the significant strides made by generative AI in just a few short years, its future progress is constrained by the challenge of building modular and robust systems. This capability has been a cornerstone of past technological revolutions, which relied on combining components to create increasingly sophisticated and reliable systems. Cars, airplanes, computers, and software consist of components-such as engines, wheels, CPUs, and libraries-that can be assembled, debugged, and replaced. A key tool for building such reliable and modular systems is specification: the precise description of the expected behavior, inputs, and outputs of each component. However, the generality of LLMs and the inherent ambiguity of natural language make defining specifications for LLM-based components (e.g., agents) both a challenging and urgent problem. In this paper, we discuss the progress the field has made so far-through advances like structured outputs, process supervision, and test-time compute-and outline several future directions for research to enable the development of modular and reliable LLM-based systems through improved specifications.

==> conclusion.tex <==
\section{Summary}

Engineering disciplines, including software engineering, have been responsible for driving staggering economic progress since the start of the industrial revolution. In this document, we contend that this progress was enabled by five key properties: verifiability, debuggability, modularity, reusability and automatic decision making. The first two properties enable developers to quickly build systems from scratch, the next two properties enable developers to build new complex systems from (existing) simpler ones, and the last property enables developers to build systems that require no human intervention. Altogether, these properties have enabled an exponential growth of the ecosystem which ultimately fueled economic growth.

Further, we argue that the key to enable these engineering properties is the ability to have clear, unambiguous specifications that precisely describe the behavior of each system component, including its output, given a particular input. 

AI, and in particular LLMs, places us on the cusp of another economic and social revolution. However, we observe that the specification of most LLM tasks are ambiguous, as they use natural language. While natural language makes LLMs widely accessible and general (i.e., anyone can describe any task), its inherent ambiguity makes it difficult to build new, more powerful systems from (existing) simpler ones, which ultimately hampers the ecosystem and economic growth.

To address this limitation, we argue for developing new techniques that make it easier to write unambiguous specifications and to verify that an LLM system implements correctly a task according to its specification, and debug the LLM system if it fails to correctly implement this task. By doing so, we can support all five software engineering properties, and enable developers to accelerate the development of new LLM solutions. solutions that are more powerful and reliable, and which can address a growing number of use cases.

